Signed, Sealed,... Confused: Exploring the Understandability and Severity of Policy Documents

In general, Terms of Service (ToS) and other policy documents are verbose and full of legal jargon, which poses challenges for users to understand. To improve user accessibility and transparency, the "Terms of Service; Didn't Read" (ToS;DR) project condenses intricate legal terminology into summaries and overall grades for the website's policy documents. Nevertheless, uncertainties remain about whether users could truly grasp the implications of simplified presentations. We conducted an online survey to assess the perceived understandability and severity of randomly chosen cases from the ToS;DR taxonomy. Preliminary results indicate that, although most users report understanding the cases, they find a bias towards service providers in about two-thirds of the cases. The findings of our study emphasize the necessity of prioritizing user-centric policy formulation. This study has the potential to reveal the extent of information imbalance in digital services and promote more well-informed user consent.

==> documentBody/OLD-RQ4results.tex <==
\section*{Results RQ4 - How did demographic traits affect understandability and severity?}
%\label{secRQ4} %Commented since section is defunct

\FIXME{JED@SSN, JED@SNS: For R2-4, we basically swap out this section for a comparative one. Be cognizant of R2-5 and provide signposting and summarization of argumentation structure at the beginning and R3-7's concerns about muddled results.
\\ SSN @JED, @SNS: So far this section expands on the descriptive stats of the demo traits. We haven't touched on how it affects U \& S.
Either we can rename this section and create a new one with U \& S, or just include the box plots here and expand. Please advise\\
JED: the current hypothesis testing section is intended to mostly REPLACE this section. It seems we added some citations, so we should put those in the aforementioned new results section, another results section, or the new discussion. Am open to hybrid approach, but I think it might be hard to implement}




The survey, conducted through the Prolific platform, got responses from 500 participants\footnote{We had demographic information from the one participant whose survey response was unrecoverable.} from the United States, who came from a very diverse demographic distribution.
Based on the information we collected, we observed the following:

\paragraph{Age} 
Based on the age data, the mean age of the participants is 35.65 years, and half of the participants are below the age of 33.
The standard deviation of 11.44 indicates a considerable heterogeneity in the age distribution among the subjects.
The estimated standard error of 0.51 indicates a little margin of error in calculating the population mean, therefore indicating that the sample offers an accurate estimation of the average age of the participants.
In general, the data indicates a wide range of ages, characterised by a central trend around the early to mid-30s.
This distribution aligns with prior findings by authors in this article~\cite{lythreatis2022digital}, who noted that younger users often engage more actively with digital platforms but may undervalue privacy risks, while older users tend to exhibit higher privacy concerns due to greater awareness of potential data misuse.

\paragraph{Gender}
The gender distribution in the dataset indicates that women constitute the majority of participants, representing 52.2\% of the total sample. 
Men constitute 46.8\% of the participants, with 1\% opting not to reveal their gender. These results reflect prior work by Hoy and Milne~\cite{hoy2010gender}, who observed that women are generally more privacy-conscious and hesitant to share personal information online, while men often prioritize functionality over privacy.
%The reasonably even distribution implies a diversified composition.
%However, a small subset of individuals who choose not to disclose their gender shows that the process of collecting data is following principles of inclusion.
%In future analysis, the almost equal distribution of males and females might give significant insights into any gender-based disparities.


\paragraph{Ethnicity}
The slight majority of the participants we sampled identified as White, accounting for 57.6\%.
A total of 13.4\% of the participants identified as Black, 12.2\% identified as Asian, and 10.4\% identified as mixed race.
About 5\% reported belonging to other ethnic groups, while 1\% selected ``N/A'' and 0.4\% opted not to declare their ethnicity. These observations are consistent with Rainie and Perrin~\cite{auxier2019americans}, who documented that ethnic minorities, including Black and Hispanic populations, often express heightened privacy concerns due to systemic trust issues and prior experiences of data misuse.



\paragraph{Employment Status}
A plurality of the participants (36.6\%, 183 individuals) were engaged in full-time employment, while 17.4\% (87 individuals) were working part-time.
Approximately 14.6\% of the respondents reported being unemployed, but an equivalent amount of 14.6\% marked their status as "N/A" (which might include students, retired persons, or those who elect not to reveal their employment status). In addition, 11.2\% of the surveyed population are not currently employed, and 5.6\% are classified as "Other," which may indicate other job circumstances. The observed distribution exhibits a wide range of job statuses, with full-time workers being the most prevalent category, but also substantial representation from individuals who are not now engaged in paid employment. This aligns with Park~\cite{park2014employee}, who found that employed individuals are more likely to manage their privacy settings due to professional risks, while unemployed or part-time workers may demonstrate less engagement with privacy settings.

\paragraph{Student Status}
The bulk of the participants were not students (67.2\%, 336 individuals), while 19.6\% (98 individuals) self-identified as students.
Furthermore, 13.2\% (66 individuals) replied ``N/A.'' Livingstone and Helsper~\cite{livingstone2007gradations} similarly noted that students are often highly active online but may trade privacy for access to services without fully considering the long-term consequences of their decisions.

\input{table/6-demographic_stats}

\paragraph{Demographic Questions outlining participant attitudes, based on GenderMag Facets, as applied to privacy attitudes}
Table~\ref{table: demoStats} showcases the responses about the participants' attitudes toward privacy policies and privacy-related behaviors.
It includes 11 questions, each addressing different aspects of privacy management, ranging from motivation to read privacy policies to comfort with sharing personal information.
For each question, the table provides the mean, median, and standard deviation (SD) of responses, along with an interpretation of the results.

The analysis shows that while participants realize the importance of privacy and are somewhat proactive about privacy settings, many are not motivated to read or understand privacy policies.
For example, the mean response for motivation to read policies (Q1) is 4.08, indicating that participants are generally not inclined to invest time in reading them, though individual responses vary widely. This aligns with findings by Acquisti et al.~\cite{acquisti2015privacy}, who showed that the length and complexity of privacy policies discourage users from reading them.
Similarly, participants are moderately confident in their ability to manage privacy settings (Q4) and feel that control over personal information is important (Q6), with relatively lower variability in responses for these items. 
These findings are consistent with Trepte et al.~\cite{trepte2011privacy}, who found that while users value control over their data, their actual knowledge of privacy settings often falls short.

The table also highlights a general discomfort with sharing personal information online (Q8) and a tendency to accept terms and conditions without reading them (Q9), corroborating prior work on user behaviors regarding privacy management.
The authors in this research~\cite{gross2005information} similarly noted that most users are hesitant to share sensitive data but frequently bypass terms and conditions due to convenience.

\paragraph{Negative experiences}
Figure~\ref{figNegExp} highlights the various categories of adverse experiences encountered by participants, indicating that the most commonly reported concern was the receipt of advertisements, impacting 274 individuals.
This is followed by data breaches reported by 223 participants.
Additional concerns, including unforeseen charges, data exploitation, and account breaches, impacted a considerable number of participants.
Account suspensions were the least prevalent adverse experience, reported by only 70 participants. These results align with findings by Martin and Murphy~\cite{martin2017role}, who noted that targeted advertisements and data breaches are among the most visible and frustrating outcomes of inadequate data privacy practices.
Figure~\ref{figNegMult} depicts the allocation of participants according to the frequency of negative experiences they faced, indicating that most participants encountered either one or two negative incidents.
The proportion of people indicating three or more adverse events consistently declines, with a mere 1\% reporting eight or nine occurrences.
Notably, 4\% of individuals reported no adverse events.
This aligns with findings by Solove~\cite{solove2012introduction}, who documented that privacy breaches are increasingly common but often concentrated among a subset of highly affected users.
\input{figure/3-negativeExp}
\input{figure/4-negativeMult}






==> documentBody/Results_SSN.tex <==
\section{Results - LOOKING FOR A HOME. We need to mine this and locate within the RQ framework provided}

\subsection{Correlation Matrix of Demographic Data}

\begin{table*}[htb]
    \centering
    \begin{tabular}{@{}lc|cc|cc@{}}
     \textbf{Question} & \textbf{Age} &
     \textbf{Gender} &\textbf{Ethnicity} &
     \textbf{Student Status} & \textbf{Employment}
     \\\hline
     \ 1 &-0.05 &	-0.04 &	0.01 &	-0.07	& 0.06
     \\\hline

     \ 2 & -0.05	 &-0.06	 & 0.05	& -0.06 & 	0.08 
     \\\hline
     
     \ 3 &  -0.01	& 0.04	& 0.01	& -0.01 &	0.07
     \\\hline
     
     \ 4 & -0.09 &	-0.04 &	0.08 &	-0.02 &	0.13 
     \\\hline
     
    \ 5 & 0.04 &	-0.08 &	0.02 &	0.00 &	-0.01
    \\\hline

    \ 6 & -0.06	& -0.05&	-0.01&	-0.09&	-0.02
    \\\hline

    \ 7 & -0.05&	-0.02&	0.00&	0.00&	0.08
    \\\hline
    
    \ 8 & 0.00	&0.05 &	0.00 &	0.09 &	0.00
\\\hline
    \ 9 & -0.01	& -0.05	& -0.01	& -0.01 &	0.01
    \\\hline
     \ 10 & -0.04	&-0.10 &	0.02&	-0.01 &	0.07
    \\\hline 
    \ 11 & -0.13	&-0.01	&0.02&	-0.05&	0.02
    \\\hline
    \end{tabular}
    \caption{Correlation Matrix of Demographic Data}
    \label{table:caseF1}
\end{table*}

Younger participants typically have higher levels of privacy awareness and proactivity, displaying stronger motivation to read privacy regulations, greater confidence in understanding and controlling privacy settings, and a greater interest in educational materials compared to older participants.
Women exhibit a moderately higher level of caution compared to men, especially when it comes to their motivation to read privacy policies, their investment of time in comprehending them, and their willingness to take action if a privacy policy raises concerns.
The influence of ethnicity on privacy views is minimal or insignificant, as most correlations indicate little to no discernible variations among different ethnic groups.
Employed persons exhibit greater prudence and proactivity towards privacy, displaying higher motivation to adhere to policies, greater confidence in controlling settings, and a higher likelihood of taking action when privacy issues emerge.
Students typically exhibit lower levels of motivation to peruse privacy regulations, perceive less significance in managing personal information, yet feel more at ease divulging personal data to internet businesses.
The level of proactivity shown by employed and younger individuals in routinely updating their privacy settings is somewhat higher, which indicates their higher level of involvement with data protection policies.
Males and older participants exhibit more ease in utilizing privacy protection protocols like VPNs, but females seem to have lower familiarity with such technology.
The younger participants exhibit a notably greater inclination to acquire further knowledge regarding privacy resources, which indicates their aspiration to have a deeper understanding of the potential hazards and safeguards accessible to them.
Although males exhibit a slightly higher level of comfort in sharing personal data, the influence of gender on sharing activities is negligible, since comfort levels generally remain similar between genders.
Differences in status between students and non-students have minimal impact on the level of proactivity in upgrading privacy settings.
Neither age nor gender significantly affects whether persons accept terms and conditions without reading them.
The employment status systematically has a favorable impact on privacy behaviors, most likely attributed to heightened exposure to data privacy policies in the professional environment.
The influence of ethnicity on attitudes towards privacy is minimal, as most correlations indicate very little to no substantial variations in behavior among different ethnic groups.
In general, younger persons exhibit a greater inclination towards proactivity and caution about privacy issues (e.g., Q4, Q7), express a higher level of interest in acquiring knowledge about privacy (Q11), and are more inclined to engage in taking action (Q10).
Women exhibit a slightly higher level of prudence and worry in several areas, including a greater inclination to peruse privacy policies (Q1), dedicate effort to comprehending them (Q2), and respond promptly when they are a cause for concern (Q10).
Although not explicitly acknowledged in the statistics, it is usually observed that more education tends to result in increased awareness and proactive conduct, as indicated by historical patterns.
\subsection{Understandability and Severity Matrix}

\begin{table*}[htb]
    \centering
    \begin{tabular}{@{}lc|cc|cc@{}}
     \textbf{Understandability Score} & \textbf{Count} &
     \textbf{Average Severity} 
     \\\hline
     \ 1 &124 &	4.02 
     \\\hline

     \ 2 & 97	 &5.38	  
     \\\hline
     
     \ 3 &  84	& 5.23	
     \\\hline
     
     \ 4 & 96 &	4.96  
     \\\hline
     
    \ 5 & 165 &	5.76
    \\\hline

    \ 6 & 157	& 5.72
    \\\hline

    \ 7 & 296 &	5.86
    \\\hline
    
    \ 8 & 350	&6.02
\\\hline
    \ 9 & 336	& 6.10
    \\\hline
     \ 10 & 790	&6.33
    \\\hline 
   
    \end{tabular}
    \caption{Understandability and Severity Matrix}
    \label{table:caseF1}
\end{table*}

The statistical analysis reveals a direct correlation between comprehensibility and seriousness. For lower scores of understandability (1 to 4), the average severity varies between 4.02 and 4.96, indicating that less comprehensible material may result in reduced perceived severity. As the understandability score grows, the average severity levels consistently rise peaking at 6.33 for the greatest understandability score of 10. The observed pattern indicates that more explicit information enables participants to more effectively understand the gravity of problems, resulting in increased assessments of severity. In summary, when the comprehensibility of material improves, the perceived seriousness of problems also rises.






==> documentBody/ReviewsCHI.tex <==
\section*{1AC review (reviewer 4)}

Expertise

Knowledgeable

Originality (Round 1)

High originality

Significance (Round 1)

Medium significance

Research Quality (Round 1)

Low research quality

Recommendation (Round 1)

\textbf{I recommend Revise and Resubmit}

1AC: The Meta-Review

In this submission, "Signed, Sealed,... Confused: Exploring the Understandability
and Severity of Policy Documents", the authors use survey methods to
examine how well people understand terms of service documents. Reviews
generally praised the originality and potential significance of this
study. However, there were several concerns as well, which would need
to be addressed before that significance can be realized. Thus, I am
recommending Revise and Resubmit.

I'll summarize the suggestions here, but the authors are encouraged to read each
review in full:

1) The limitations of the Prolific sample should be taken more seriously,
particularly with regard to claims about "laypersons" (2AC)
2) The framing of the question "Which party does this case tend to favor?"
appeared to be confusing, and may require additional explanation (2AC)
3) All three reviewers had concerns about presentation clarity and organization,
including the introduction (R1), literature review (R1, R3), results
(2AC), and discussion (R3). The reviewers all had helpful suggestions
for how to improve the structure of this submission, which I suggest
the authors consider.
4) Potentially related to the above, the contribution of this work to the HCI
community needs to be clarified, and perhaps a more critical
consideration of the fact that ToS documents are, generally speaking,
largely designed to favor the service provider would help frame the
results (R1)
5) There were several concerns about the analysis, including the sample size, lack
of inferential statistics, and questions/claims that appear out-of-
scope given the methods used (R1).

Overall, the reviewers generally saw potential in this work, but I would encourage
the others to take these suggestions (particularly those related to
writing, framing, and methods) seriously; my impression is they are
all critical in evaluating the contribution of the work.

----------------------------------------------------------------

\section*{2AC review (reviewer 2)}

Expertise

Expert

Originality (Round 1)

High originality

Significance (Round 1)

High significance

Research Quality (Round 1)

High research quality

Contribution Compared to Length (Round 1)

The paper length was commensurate with its contribution.

Figure Descriptions

The figure descriptions are adequate and follow the accessibility guidelines.

Recommendation (Round 1)

\textbf{I recommend Revise and Resubmit}

Review (Round 1)

Summary: This paper describes the results of an online survey aimed at assessing
how Internet users understand the presentation of content from Terms
of Service documents.

Originality and Prior Work: The current draft makes a strong case that the survey
instrument designed for the study can provide a novel perspective on
the "Privacy Paradox" and past findings on the privacy decision-
making, the economics of digital privacy, etc. Overall, I think there
is a strong novel contribution here. The coverage of related work here
is quite reasonable. 
\hl{R2-1: While there is a body of work that might also be
relevant to discuss (one example below), I think the current amount of
coverage and specificity is already reasonable.}
\FIXED{Add the citation
\\SNS: Citation added in main.bib. Will add in the text as appropriate\\
JED: located in section 2, though it may move to 1.}

Goldfarb, A. and Que, V.F., 2023. The economics of digital privacy. Annual Review
of Economics, 15(1), pp.267-286.

Significance: I think this paper stands to have high potential impact. The topic
is generally relevant to a large portion of the HCI field, which
increasingly involves online platforms in some capacity (arguably the
growth of AI-related research in HCI will make this work, and follow
up work, even more important).
\FIXED{Consider stealing some language from the above for our conclusion\\
JED: located in conclusion}


Research quality: The presented research decisions are all reasonably well
justified. There are a few opportunities for improvement that may
impact how seriously readers take the study.
\hl{R2-2: * The Prolific-only sample is likely to skew results somewhat towards a more-
online population. I'm not sure the current results really reflect
"laypersons" as claimed, but nonetheless are still very important.
While not a major issue, highlighting the importance of follow up work
on a more general audience could be useful as a minor edit. This
weakness is mentioned (8.2) but I think could be taken more seriously
in future drafts.
}
\FIXED{Writing issue, weaken the "laypersons" claim, move up the limitation. Not really sure what it would mean to take this more seriously.
\\SNS: Seems more like demanding a distinction between experts vs others (laypersons)\\
JED: placed in the introduction, at first usage}
\hl{R2-3: * I was a little confused at first about the "What party does this case tend to
favor?" framing; this just didn't necessarily seem like an intuitive
way people might think about the Terms of Service for the platforms
discussed in motivating paragraphs. I did look at the supplement
materials (data) which was helpful, but still was left thinking the
paper could benefit from more explanation of this framing and what
this implies for user-platform interactions in general.
}
\FIXED{We need to hit this cleanly, in that we need to clarify what this means while still staying faithful to what participants saw\\
JED: located in Section 3}

* The understandability results were all very clear throughout.

Presentation clarity: In terms of writing quality and results tables, the paper
was clear throughout. \hl{R2-4: The results might benefit from visualization
rather than mean and standard deviations of ordinal responses.}
\FIXED{Add boxplots and maybe statistical testing
\\SNS: Sameer will be working on this\\
JED: located in Section 7, which we will rewrite fully}
\hl{R2-5: The
results section could benefit from a bit more signposting (while a
reader who has read the first 3 sections already has a pretty decent
picture of the survey itself in their mind and thus how the results
might be presented, a quick summary of Section 4 and 5's organization)
could be beneficial.}
\FIXED{Basically just follow the advice in the last part of this WHILE being wary of oversummarization\\
JED: located in all results sections}

In summary, this paper is strong throughout. 
\hl{R2-2 (again): My main concerns are that the sample
doesn't quite match some of the claims in the Introduction and
Discussion about speaking to layperson perceptions (acknowledged in
limitations)}
and some of the framing of these survey questions could
be confusing. That said, most of the results are explained well and
the implications are relatively clear.

I look forward to seeing future iterations of this paper.

----------------------------------------------------------------

\section*{reviewer review (reviewer 1)}

Expertise

Knowledgeable

Originality (Round 1)

Medium originality

Significance (Round 1)

Low significance

Research Quality (Round 1)

Low research quality

Contribution Compared to Length (Round 1)

The paper length was commensurate with its contribution.

Figure Descriptions



Recommendation (Round 1)

\textbf{I can go with either Reject or Revise and Resubmit}

Review (Round 1)

Summary:
This paper presents a user study of the comprehensibility of elements from terms
of service. The project is based on the "Terms of Service; Didn't
Read" (ToS;DR) project, which digests terms of service documents into
sets of standardized elements and assigns ratings from A to E based on
their content. The authors had  499 crowdworks each to review a random
set of 5 of the TOS;DR policy elements (termed "cases"), asking them
to provide likert scale ratings of understandability and the severity
of perceived favoritism (termed "severity") towards the service
provider or user. The authors use descriptive statistics to analyze
the understandability and severity of different policy elements.

Comments:
I thank the authors for their submission to CHI 2025. I appreciate the hard work
that clearly went into conducting this study, and recognize that it
presents an original idea. Nevertheless, I cannot recommend accepting
this paper in its current form due to a general lack of structure
which inhibits its clarity,  an unclear contribution, and the need for
better justification of the methods. Please see my detailed comments
on each below:

**General lack of structure**
I think it is necessary to discuss this issue first, as it is pervasive and feeds
into the other major issues I have. 
\hl{R1-1: Most sentences are well written,
but the paper lacks an overall structure which makes it difficult to
comprehend for the reader.}
\FIXED{best fixed via boldify/outline kind of exercises. Added TODO}
For example, the 
\hl{R1-2: introduction provides some
useful background information, but lacks an outline of the paper or
other signposting that is typical in an academic paper (e.g.,
description of methods, explanation of the results, list of sections
and their purpose, etc.)
}
\FIXED{Not going to list sections and their purpose, but we can do the rest of this. Located in introduction}
The research questions are abruptly
introduced with expected contributions, with no other details provided
about the study to come.

\hl{R1-3: Similarly, the related work begins to discuss background information without a
clear indication of why the authors are discussing this particular
research. For example, it is unclear to me why there is a social media
subsection. There are also no summarizing statements about how a
particular research area relates to the present study or why the
present study is unique from the other studies in this area (e.g.,
"Our study builds upon social media research by Y" or "No prior study
has done X"). As a result, the related work section reads like a
largely self-contained annotated bibliography.}
\FIXED{We can lightly position ourselves with respect to this work. I generally don't like justification for the chosen method appearing in the related work, but this reviewer seems to want it, so we can move in that direction (but I would recommend against pulling TOO MUCH of that type of content into related work).\\
Positioned in background}

This lack of scaffolding is evident beyond these two sections, but I will leave it
here for brevity's sake. These types of writing issues could be
addressed in a revision, although substantial revision is necessary.

**Lack of clear contribution**
\hl{R1-4: A more fundamental issue I have with the study is that I do not really understand
the motivation for conducting it or what contribution it provides. The
main takeaways seem to be that the cases from TOS;DR are 1) generally
considered comprehensible by users (with some exceptions) and 2)
favorable to services. Beyond, maybe, helping to improve TOS;DR, the
first finding seems to have limited utility to the broader HCI
community. Perhaps there is some conclusion to be drawn about what
elements of terms of service are particularly confusing, but most
users are not referring to ToS;DR (or really any website policy
document). It is therefore unclear how this insight is useful. This
second finding seems almost tautological, as terms of services largely
exist to curtail users' rights.}
\FIXED{They are correct in terms of 1+2, though I would add a third thing, which will come from the comparative stats.
The main fix here is that we need to clarify to them how folks can use 1+2. Tn particular, for \#1, one method to improve understanding of these docs could be discovering instances of these critical concepts (e.g., with classification) and since we know they are understandable. For \#2, this then lets us perform triage, since now we know which concepts user care more/less about.\\
Located in discussion for now (Fixes should appear in a mix of places)}

This issue may be solved by fixing the problems with writing. 
\hl{R1-5: In particular, any
future revision should clarify why it is important to investigate the
understandability of ToS;DR cases, beyond the fact that it is a
standard database.}
\FIXED{Clarify as described, in introduction}
\hl{R1-6: The authors should also make it clear what these
results mean and what implications they have for the issues raised in
the introduction, like the privacy paradox and unexpected elements in
privacy policies.
Adding a discussion section could be a good place
for the analysis of the broader implications.}
\FIXED{We can add a discussion section as requested}

**Insufficient  methods**
The final major issue I have with the study is that I believe the methods are not
well justified and, at times, insufficient to answer the research
questions as currently stated.

\hl{R1-7: First, I think there is an issue with sample size. 499 seems like a sufficient
sample size to draw macro conclusions (i.e, that the set of cases is
generally understandable) but the between case comparisons seem more
dubious.  It is, of course, impossible to show all participants each
of the 243 case definitions, but this means that only a small number
of participants saw each condition. 499/(243/5) = ~10 each. I am glad
the authors raise this issue in the he threats to validity section.
This design may be acceptable, but I think justification is necessary
(i.e., citation to relevant literature with similar design).}
\FIXED{ Located in methodology.
This one is a little thorny... Possible we just ignore, possible we expand that threats. I do not know of similar designs and would not really want to, e.g., triple the sample size so that we get CLT in between-case comparison (that doesn't seem necessary to me since we aren't drawing statistical conclusions of that kind, trying to light pathways for more targeted study of particular concepts)}

\hl{R1-8: The study also relies on interpreting descriptive statistics to draw its
conclusions. No statistical testing was performed to validate that the
differences between cases in understandability or severity were
significant. Statistical testing is not always necessary nor
appropriate, but the descriptive analysis seems, at points, highly
subjective and arbitrary. No defined procedure is explained in methods
nor is a reference cited to justify this approach.  A particular area
of concern for me is section 6. The authors initially find no
correlation between understandability and severity, but nevertheless
go onto crop the data in different ways to try to draw conclusions
(i.e., looking at the most and least understandable/severe alone).
Ultimately, I'm left with really no takeaways from this section.}
\FIXED{Located in the New RQ4 section\\
And here we get yelled at for the expected reason. Replace that section with a better one relying on comparative
\\SNS: Sameer will be working on improving the stats altogether.
\\
SSN: Will resume working on the stats after addressing some comments and come up with a concrete response.}

\hl{R1-8: (mostly duplicated) Research question 4 ("How did demographic traits affect understandability and
severity?") also seems to be unanswerable with the paper's descriptive
approach. It is valuable to contextualize the other results by
describing the characteristics of the participants, but no analysis is
discussed to determine whether the demographics are associated with
understandability or severity. The authors do not even hypothesize
about how the demographics may effect the results. This research
question is, therefore, left unaddressed.}
\FIXED{Same treatment. Very similar to previous point, but slightly more targeted
\\ 
SSN: New hypotheses have been added to tackle this comment.}

Ultimately, any revision of the paper should better justify the methodological
approach, especially with respect to the sampling approach and the
reliance on seemingly non-systematic descriptive statistics. The
procedure and \hl{R1-9: choices to crop the data in certain ways should be
justified.}
\FIXED{JED@SSN: I think this goes away as a knock on when swapping in comparative stats, but seems related to their criticism of section 6.1}

**Misc other issues**
What follows is a list of other issues that I noticed during my reading, which I
think should be addressed in any revision.

\hl{R1-10: 1: The research questions use terminology before it has been defined in the paper
like  "understandability data" or "severity data."}
\FIXED{define these terms, I guess? seems fairly obvious, but we can probably add clarity
\\SNS: Will clarify to ensure there is no confusion\\
located in introduction}
\hl{R1-11: In general, the
narrow phrasing of the research questions is not very useful.}
\FIXED{See if we can broaden., located with RQs}
\hl{R1-12: 2: Throughout related work, papers are summarized or quoted without reference to
what the research did or the context of the results. This makes it
difficult for a reader to evaluate the synthesis. E.g., "Slightly over
half of participants (51\%) felt that information about their general
searching activities,... impacts their feelings about tracking." [26]
=> What context is this quote from? What is the information referred
to about general searching activities? "According to Earp et al. [15],
people are more likely to read and understand privacy regulations when
they believe that their data is in grave danger." => How did they draw
that conclusion? What is the context?}
\FIXED{This is fairly typical, I am not sure what they really want here, since doing this consistently costs a LOT of words (and will make things more boring). Might ignore... still thinking. located in background}
\hl{R1-13: 3: Line 216: "To determine the set of concepts the participants would see, as well
as the text to represent each concept, we appeal to Terms of Service;
Didn't Read (ToSDR) [38]." At this point in the paper, ToSDR is not
well introduced. I am left with the questions: What is ToSDR? What
does it contain? Why is it a reasonable source for this purpose? What
are cases? Are they like parts of a policy?}
\FIXED{Answer these questions just in time in the intro}
\hl{R1-14: 4: Footnotes are not an appropriate citation (E.g., footnote 5 and 6). If linking
to a live website or service, a footnote makes sense.  See:
https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.acm.org%2Fpublications%2Fauthors%2Freference-formatting&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203068419%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=Kq%2BI2YscHLnCoMT5nk7b41pJbvrxqPx7vvMtcsMWl%2Bo%3D&reserved=0
}
\FIXED{Fine, fix them, passing over this for now since I need to look at all our footnotes. TODO added}
\hl{R1-15: 5: Line 302: "However, there is no significant correlation (Pearson's correlation
t-test, t(2498) = 6.99, p = 3.45 e-12) between understandability and
severity." 1. There is no such thing as "Pearson's correlation
t-test,"  2. The p-value appears very small and significant under most
normal interpretations. Later in the paper, the opposite is stated:
"we see that higher understandability scores tend to result in a rise
in the mean severity score." (line 618). Which is true? Or are the
supposed to mean different things?}
\FIXED{JED@SSN: Can you assist with chasing this out?. TODO added}
\hl{R1-16: 7: Page 7: table is in the footer.}
\FIXED{doesnt seem possible, but we should check our layout for this when submitting revision. Audit added}
\hl{R1-17: 8: The question that is the title of 4.2 is not addressed in the subsection. Was
any analysis performed to actually tell if participant written
explanations are better?}
\FIXED{No, we need to set expectations differently here. Located in that section}
\hl{R1-18: 9: line 748: Why is the 500th participant included in demographic calculations if
their other data is not used? They are functionally not part of the
study.}
\FIXED{JED@SNS: I need help disentangling this. I recall we had trouble identifying WHICH responses didn't belong when faced with a few sums that didnt agree\\
TODO added}
\hl{R1-19: 10: The privacy paradox is discussed in the introduction, but never returned to.
Why is this relevant?}
\FIXED{Add a discussion, as requested}
\hl{R1-20: 11: There is no complete listing of the survey available to reviewers. This makes
it challenging to evaluate the methods. It is generally best practice
to include the survey instrument in the appendix.}
\FIXED{Provide the word document and redacted link. TODO added}
\hl{R1-21: 12: The entire subsection 6.1 is confusingly written. Its unclear which responses
are being discussed when. What do the numbers 110 and 35 reports
correspond to? I can infer somewhat, but it's not clear.}
\FIXED{I also didn't find these parts very compelling. It could be we chop (or condense) it to make room for a deeper comparative stats treatment in a roughly space-neutral way\\
JED@SNS, JED@SSN, what do you think?
\\ 
SSN: In order to clarify this, we can rephrase it better (for lack of a better term, dumb it down)
Basically start with what is meant by least understandable, and how many responses suggest the same. Then from there, since all 110 responses suggest that the case(s) were least understandable,  35 responses suggest that they were very severe (< -5). The explanation seems to make sense. Then, 7/110 responses had the highest severity rating. 
If needed, we can do the same thing for 6.1 - 6.4\\
Located in section 6/RQ3}
\hl{R1-22: 13: Gender subsection of section 7 suggests that only binary gender options were
presented. This is against best practice. See https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.morgan-%2F&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203088867%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=xBp%2FMwXRYkf%2FQ2hpCVIqnSTVHoH7O51Oe7P05jN39JE%3D&reserved=0
klaus.com/gender-guidelines.html}
\FIXED{We complied with this, but did not state as much. Another reason to show the instrument\\ Located in methodology}
\hl{R1-23: 14: The questions adapted from GenderMag do not seem to me to be appropriately
called demographics. They seem more like privacy attitude/behavior
questions.}
\FIXED{Fine, whatever. Audit added}
\hl{R1-24: 15: section  8.2 on external validity should discuss the characteristics of
Prolific crowdworkers. See Tang et al. https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.usenix.org%2Fconferen&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203109173%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=DD6uUBpBwdKjY8CV4vfJwnPV%2BKTO%2B9wZdqe7B9kdYQw%3D&reserved=0
ce/soups2022/presentation/tanghttps://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.usenix.org%2Fconference%2Fsoups2&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203128203%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=g1ut9Nd7jG3NgDohw2AxoxnTs6BngWDLmvHkihZ62Uo%3D&reserved=0
022/presentation/tang}
\FIXED{Add the citation, located in threats}
\hl{R1-25: 16: how was the sample size determined? Was power analysis performed?}
\FIXED{No, power analysis is a waste of time. If i recall, we wanted around 10 responses to each case, since that would give a reasonable estimate of mean+SD. We were not intending to draw comparative statistics across cases, which we could barebones at 15 responses to each case. However, that would increase the cost by 50\%\\
JED: located in section 3}
\hl{R1-26: 17: The title suggests that the authors found that the policies were confusing,
but they were largely understandable.}
\FIXED{Good point, we can sharpen the conclusion with this. Basically say that we found participants could understand the individual concepts, while prior work has consistently shown inability to understand whole policies. Therefore, extracting concepts via classification shows promise.\\
JED: located in conclusion}

----------------------------------------------------------------

\section*{reviewer review (reviewer 3)}

Expertise

Expert

Originality (Round 1)

Medium originality

Significance (Round 1)

Medium significance

Research Quality (Round 1)

Medium research quality

Contribution Compared to Length (Round 1)

The paper length was commensurate with its contribution.

Figure Descriptions

The figure descriptions are adequate and follow the accessibility guidelines.

Recommendation (Round 1)

\textbf{I recommend Revise and Resubmit}

Review (Round 1)

Thank you for your submission, I enjoyed reviewing your paper. You take up
important, timely research questions on the understandability of
privacy policies. I found your research questions to be original, and
your methods sound and rigorous. It is great, for example, to have
empirical work that shows which privacy concepts are "understandable"
and your tables and descriptions show a great amount of detail.

That being said, I do have a number of concerns (e.g. related works, discussion /
implications) and presentation clarity that in the current state
obstruct the impact of this work.

Overall, 
\hl{R3-1: I find that this paper could be written more clearly. It could use a few
rounds of heavy copy editing to ensure a smoother flow.}
\FIXED{Spend some time doing copy editing and such. Boldifies constructed retroactively might help too\\
JED: Audit added}

Next, I find that our 
\hl{R3-2: paper is not sufficiently motivated in the introduction}
\FIXED{Audit this, boldifies will probably help}
, nor
\hl{R3-3: sufficiently grounded adequately in prior work}
\FIXED{Add whatever citations they provide. If they don't give guidance, probably ignore}
. For example, you
present your research questions in the introduction without defining
the research area — 
\hl{R3-2 (again): what is "understandability data"? What are the
privacy concepts that ToSDR encompasses? Why is this your research
site?}
\FIXED{JED: located in introduction}

Related Works:

While your related works section does an adequate job of citing prior works - 
\hl{R3-4: I
find the organization unconvincing and the subsections scattered. It
would strengthen your paper to rewrite this section with a better
flow.
For example, you start this section with:

Websites profit off
people's trust by selling, sharing, or analyzing personal information
[39]. As an example of the effects
of these behaviors, "Slightly over half of participants (51\%) felt that
information about their general searching activities,...impacts their
feelings about tracking." [26]. 

This does not read well. Summarizing
the quote would be a better approach.
}
\FIXED{Not sure, would need to read it\\
JED: located in background}
\hl{R3-5: Further as some more general
writing tips, please use topic sentences and work on the transition
flows between paragraphs and new ideas.}
\FIXED{Audit created, improve as able}

Here are some more concrete suggestions towards a more organized structure for
your related works section:

\hl{R3-6: 1. Starting the section with an overview of a privacy theory or framework you are
using and how you define privacy policies. You should ground these in
related works in the HCI space.}
\FIXED{Not fully sure what we do here either, since I do not know much about privacy frameworks\\
JED: located in background}
\hl{2. A subsection that starts with outlining the problem spaces concerning privacy
policies (and then continuing with the other subsections you have).}
\FIXED{This seems somewhat reasonable, but I am not sure I can adequately articulate this problem space\\
JED: located in background}

You cite the contextual integrity framework, which is fantastic. Along these
lines, I would urge you to review this robust Zotero library for more
work: \url{https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.zotero.org%2Fgroups%2F2228317%2Fprivaci%2Flibrary&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203255851%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=kuZvZm3fJMA%2FAtB4ogZvTzz3wauECQHegKaWaY0kpho%3D&reserved=0} but
especially \hl{R3-6 (cont'd: Shvartzshnaider et al., "Going against the (appropriate)
flow: a contextual integrity approach to privacy policy analysis".}
\FIXED{Check out these resources\\
JED: located in background}

Discussion / Implications

\hl{R3-7: Your findings and implications sections are quite muddled and it is very
challenging to follow. I would highly recommend combing through these
sections and trying to rewrite this for flow and readability.}
\FIXED{Same treatment as above\\
JED: located in al results sections}
\hl{R3-8: Importantly, throughout these sections, please cite prior work from
your related works section. Here, you should be articulating how prior
research informs (builds on, supports, or discounts, etc.) your
empirical contributions -- this is crucial for having a paper with
strong impact.}
\FIXED{Need to rely on Shikha to foreground these concepts\\
JED: located in all results sections}

I look forward to reviewing your edits. Good luck!

\FIXED{I have adjusted for the following copy edit}
Other specific edits:

Introduction:

Period missing at the end of second bullet point under "By answering these RQs, we
make the following contributions"

Methodology:

Introduction is needed for ToSDR - what is ToSDR? Why ToSDR? What is the object or
unit of analysis when scraping ToSDR?

Period missing at the end of the last sentence in section 3.1 (Demographic
information)

Findings / Implications / Discussion:

Period missing at the end of the last sentence in section 4.3

----------------------------------------------------------------



==> documentBody/ReviewsCHIorig.tex <==
1AC review (reviewer 4)

 Expertise

   Knowledgeable

 Originality (Round 1)

   High originality

 Significance (Round 1)

   Medium significance

 Research Quality (Round 1)

   Low research quality

 Recommendation (Round 1)

   I recommend Revise and Resubmit

 1AC: The Meta-Review

   In this submission, “Signed, Sealed,... Confused: Exploring the Understandability
               and Severity of Policy Documents”, the authors use survey methods to
               examine how well people understand terms of service documents. Reviews
               generally praised the originality and potential significance of this
               study. However, there were several concerns as well, which would need
               to be addressed before that significance can be realized. Thus, I am
               recommending Revise and Resubmit.

   I’ll summarize the suggestions here, but the authors are encouraged to read each
               review in full:

   1) The limitations of the Prolific sample should be taken more seriously,
               particularly with regard to claims about “laypersons” (2AC)
   2) The framing of the question “Which party does this case tend to favor?”
               appeared to be confusing, and may require additional explanation (2AC)
   3) All three reviewers had concerns about presentation clarity and organization,
               including the introduction (R1), literature review (R1, R3), results
               (2AC), and discussion (R3). The reviewers all had helpful suggestions
               for how to improve the structure of this submission, which I suggest
               the authors consider.
   4) Potentially related to the above, the contribution of this work to the HCI
               community needs to be clarified, and perhaps a more critical
               consideration of the fact that ToS documents are, generally speaking,
               largely designed to favor the service provider would help frame the
               results (R1)
   5) There were several concerns about the analysis, including the sample size, lack
               of inferential statistics, and questions/claims that appear out-of-
               scope given the methods used (R1).

   Overall, the reviewers generally saw potential in this work, but I would encourage
               the others to take these suggestions (particularly those related to
               writing, framing, and methods) seriously; my impression is they are
               all critical in evaluating the contribution of the work.

----------------------------------------------------------------

2AC review (reviewer 2)

 Expertise

   Expert

 Originality (Round 1)

   High originality

 Significance (Round 1)

   High significance

 Research Quality (Round 1)

   High research quality

 Contribution Compared to Length (Round 1)

   The paper length was commensurate with its contribution.

 Figure Descriptions

   The figure descriptions are adequate and follow the accessibility guidelines.

 Recommendation (Round 1)

   I recommend Revise and Resubmit

 Review (Round 1)

   Summary: This paper describes the results of an online survey aimed at assessing
               how Internet users understand the presentation of content from Terms
               of Service documents.

   Originality and Prior Work: The current draft makes a strong case that the survey
               instrument designed for the study can provide a novel perspective on
               the “Privacy Paradox” and past findings on the privacy decision-
               making, the economics of digital privacy, etc. Overall, I think there
               is a strong novel contribution here. The coverage of related work here
               is quite reasonable. While there is a body of work that might also be
               relevant to discuss (one example below), I think the current amount of
               coverage and specificity is already reasonable.

   Goldfarb, A. and Que, V.F., 2023. The economics of digital privacy. Annual Review
               of Economics, 15(1), pp.267-286.

   Significance: I think this paper stands to have high potential impact. The topic
               is generally relevant to a large portion of the HCI field, which
               increasingly involves online platforms in some capacity (arguably the
               growth of AI-related research in HCI will make this work, and follow
               up work, even more important).

   Research quality: The presented research decisions are all reasonably well
               justified. There are a few opportunities for improvement that may
               impact how seriously readers take the study.
   * The Prolific-only sample is likely to skew results somewhat towards a more-
               online population. I’m not sure the current results really reflect
               “laypersons” as claimed, but nonetheless are still very important.
               While not a major issue, highlighting the importance of follow up work
               on a more general audience could be useful as a minor edit. This
               weakness is mentioned (8.2) but I think could be taken more seriously
               in future drafts.
   * I was a little confused at first about the “What party does this case tend to
               favor?” framing; this just didn’t necessarily seem like an intuitive
               way people might think about the Terms of Service for the platforms
               discussed in motivating paragraphs. I did look at the supplement
               materials (data) which was helpful, but still was left thinking the
               paper could benefit from more explanation of this framing and what
               this implies for user-platform interactions in general.
   * The understandability results were all very clear throughout.

   Presentation clarity: In terms of writing quality and results tables, the paper
               was clear throughout. The results might benefit from visualization
               rather than mean and standard deviations of ordinal responses. The
               results section could benefit from a bit more signposting (while a
               reader who has read the first 3 sections already has a pretty decent
               picture of the survey itself in their mind and thus how the results
               might be presented, a quick summary of Section 4 and 5’s organization)
               could be beneficial.

   In summary, this paper is strong throughout. My main concerns are that the sample
               doesn’t quite match some of the claims in the Introduction and
               Discussion about speaking to layperson perceptions (acknowledged in
               limitations) and some of the framing of these survey questions could
               be confusing. That said, most of the results are explained well and
               the implications are relatively clear.

   I look forward to seeing future iterations of this paper.

----------------------------------------------------------------

reviewer review (reviewer 1)

 Expertise

   Knowledgeable

 Originality (Round 1)

   Medium originality

 Significance (Round 1)

   Low significance

 Research Quality (Round 1)

   Low research quality

 Contribution Compared to Length (Round 1)

   The paper length was commensurate with its contribution.

 Figure Descriptions



 Recommendation (Round 1)

   I can go with either Reject or Revise and Resubmit

 Review (Round 1)

   Summary:
   This paper presents a user study of the comprehensibility of elements from terms
               of service. The project is based on the “Terms of Service; Didn’t
               Read” (ToS;DR) project, which digests terms of service documents into
               sets of standardized elements and assigns ratings from A to E based on
               their content. The authors had  499 crowdworks each to review a random
               set of 5 of the TOS;DR policy elements (termed “cases”), asking them
               to provide likert scale ratings of understandability and the severity
               of perceived favoritism (termed “severity”) towards the service
               provider or user. The authors use descriptive statistics to analyze
               the understandability and severity of different policy elements.

   Comments:
   I thank the authors for their submission to CHI 2025. I appreciate the hard work
               that clearly went into conducting this study, and recognize that it
               presents an original idea. Nevertheless, I cannot recommend accepting
               this paper in its current form due to a general lack of structure
               which inhibits its clarity,  an unclear contribution, and the need for
               better justification of the methods. Please see my detailed comments
               on each below:

   **General lack of structure**
   I think it is necessary to discuss this issue first, as it is pervasive and feeds
               into the other major issues I have. Most sentences are well written,
               but the paper lacks an overall structure which makes it difficult to
               comprehend for the reader. For example, the introduction provides some
               useful background information, but lacks an outline of the paper or
               other signposting that is typical in an academic paper (e.g.,
               description of methods, explanation of the results, list of sections
               and their purpose, etc.). The research questions are abruptly
               introduced with expected contributions, with no other details provided
               about the study to come.

   Similarly, the related work begins to discuss background information without a
               clear indication of why the authors are discussing this particular
               research. For example, it is unclear to me why there is a social media
               subsection. There are also no summarizing statements about how a
               particular research area relates to the present study or why the
               present study is unique from the other studies in this area (e.g.,
               “Our study builds upon social media research by Y” or “No prior study
               has done X”). As a result, the related work section reads like a
               largely self-contained annotated bibliography.

   This lack of scaffolding is evident beyond these two sections, but I will leave it
               here for brevity's sake. These types of writing issues could be
               addressed in a revision, although substantial revision is necessary.

   **Lack of clear contribution**
   A more fundamental issue I have with the study is that I do not really understand
               the motivation for conducting it or what contribution it provides. The
               main takeaways seem to be that the cases from TOS;DR are 1) generally
               considered comprehensible by users (with some exceptions) and 2)
               favorable to services. Beyond, maybe, helping to improve TOS;DR, the
               first finding seems to have limited utility to the broader HCI
               community. Perhaps there is some conclusion to be drawn about what
               elements of terms of service are particularly confusing, but most
               users are not referring to ToS;DR (or really any website policy
               document). It is therefore unclear how this insight is useful. This
               second finding seems almost tautological, as terms of services largely
               exist to curtail users’ rights.

   This issue may be solved by fixing the problems with writing. In particular, any
               future revision should clarify why it is important to investigate the
               understandability of ToS;DR cases, beyond the fact that it is a
               standard database. The authors should also make it clear what these
               results mean and what implications they have for the issues raised in
               the introduction, like the privacy paradox and unexpected elements in
               privacy policies.  Adding a discussion section could be a good place
               for the analysis of the broader implications.

   **Insufficient  methods**
   The final major issue I have with the study is that I believe the methods are not
               well justified and, at times, insufficient to answer the research
               questions as currently stated.

   First, I think there is an issue with sample size. 499 seems like a sufficient
               sample size to draw macro conclusions (i.e, that the set of cases is
               generally understandable) but the between case comparisons seem more
               dubious.  It is, of course, impossible to show all participants each
               of the 243 case definitions, but this means that only a small number
               of participants saw each condition. 499/(243/5) = ~10 each. I am glad
               the authors raise this issue in the he threats to validity section.
               This design may be acceptable, but I think justification is necessary
               (i.e., citation to relevant literature with similar design).

   The study also relies on interpreting descriptive statistics to draw its
               conclusions. No statistical testing was performed to validate that the
               differences between cases in understandability or severity were
               significant. Statistical testing is not always necessary nor
               appropriate, but the descriptive analysis seems, at points, highly
               subjective and arbitrary. No defined procedure is explained in methods
               nor is a reference cited to justify this approach.  A particular area
               of concern for me is section 6. The authors initially find no
               correlation between understandability and severity, but nevertheless
               go onto crop the data in different ways to try to draw conclusions
               (i.e., looking at the most and least understandable/severe alone).
               Ultimately, I’m left with really no takeaways from this section.

   Research question 4 (“How did demographic traits affect understandability and
               severity?”) also seems to be unanswerable with the paper’s descriptive
               approach. It is valuable to contextualize the other results by
               describing the characteristics of the participants, but no analysis is
               discussed to determine whether the demographics are associated with
               understandability or severity. The authors do not even hypothesize
               about how the demographics may effect the results. This research
               question is, therefore, left unaddressed.

   Ultimately, any revision of the paper should better justify the methodological
               approach, especially with respect to the sampling approach and the
               reliance on seemingly non-systematic descriptive statistics. The
               procedure and choices to crop the data in certain ways should be
               justified.

   **Misc other issues**
   What follows is a list of other issues that I noticed during my reading, which I
               think should be addressed in any revision.

   1: The research questions use terminology before it has been defined in the paper
               like  “understandability data” or “severity data.” In general, the
               narrow phrasing of the research questions is not very useful.
   2: Throughout related work, papers are summarized or quoted without reference to
               what the research did or the context of the results. This makes it
               difficult for a reader to evaluate the synthesis. E.g., “Slightly over
               half of participants (51%) felt that information about their general
               searching activities,... impacts their feelings about tracking.” [26]
               => What context is this quote from? What is the information referred
               to about general searching activities? “According to Earp et al. [15],
               people are more likely to read and understand privacy regulations when
               they believe that their data is in grave danger.” => How did they draw
               that conclusion? What is the context?
   3: Line 216: “To determine the set of concepts the participants would see, as well
               as the text to represent each concept, we appeal to Terms of Service;
               Didn’t Read (ToSDR) [38].” At this point in the paper, ToSDR is not
               well introduced. I am left with the questions: What is ToSDR? What
               does it contain? Why is it a reasonable source for this purpose? What
               are cases? Are they like parts of a policy?
   4: Footnotes are not an appropriate citation (E.g., footnote 5 and 6). If linking
               to a live website or service, a footnote makes sense.  See:
               https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.acm.org%2Fpublications%2Fauthors%2Freference-formatting&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203068419%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=Kq%2BI2YscHLnCoMT5nk7b41pJbvrxqPx7vvMtcsMWl%2Bo%3D&reserved=0
   5: Line 302: “However, there is no significant correlation (Pearson’s correlation
               t-test, t(2498) = 6.99, p = 3.45 e-12) between understandability and
               severity.” 1. There is no such thing as “Pearson’s correlation
               t-test,”  2. The p-value appears very small and significant under most
               normal interpretations. Later in the paper, the opposite is stated:
               “we see that higher understandability scores tend to result in a rise
               in the mean severity score.” (line 618). Which is true? Or are the
               supposed to mean different things?
   7: Page 7: table is in the footer.
   8: The question that is the title of 4.2 is not addressed in the subsection. Was
               any analysis performed to actually tell if participant written
               explanations are better?
   9: line 748: Why is the 500th participant included in demographic calculations if
               their other data is not used? They are functionally not part of the
               study.
   10: The privacy paradox is discussed in the introduction, but never returned to.
               Why is this relevant?
   11: There is no complete listing of the survey available to reviewers. This makes
               it challenging to evaluate the methods. It is generally best practice
               to include the survey instrument in the appendix.
   12: The entire subsection 6.1 is confusingly written. Its unclear which responses
               are being discussed when. What do the numbers 110 and 35 reports
               correspond to? I can infer somewhat, but it’s not clear.
   13: Gender subsection of section 7 suggests that only binary gender options were
               presented. This is against best practice. See https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.morgan-%2F&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203088867%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=xBp%2FMwXRYkf%2FQ2hpCVIqnSTVHoH7O51Oe7P05jN39JE%3D&reserved=0
               klaus.com/gender-guidelines.html
   14: The questions adapted from GenderMag do not seem to me to be appropriately
               called demographics. They seem more like privacy attitude/behavior
               questions.
   15: section  8.2 on external validity should discuss the characteristics of
               Prolific crowdworkers. See Tang et al. https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.usenix.org%2Fconferen&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203109173%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=DD6uUBpBwdKjY8CV4vfJwnPV%2BKTO%2B9wZdqe7B9kdYQw%3D&reserved=0
               ce/soups2022/presentation/tanghttps://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.usenix.org%2Fconference%2Fsoups2&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203128203%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=g1ut9Nd7jG3NgDohw2AxoxnTs6BngWDLmvHkihZ62Uo%3D&reserved=0
               022/presentation/tang
   16: how was the sample size determined? Was power analysis performed?
   17: The title suggests that the authors found that the policies were confusing,
               but they were largely understandable.

----------------------------------------------------------------

reviewer review (reviewer 3)

 Expertise

   Expert

 Originality (Round 1)

   Medium originality

 Significance (Round 1)

   Medium significance

 Research Quality (Round 1)

   Medium research quality

 Contribution Compared to Length (Round 1)

   The paper length was commensurate with its contribution.

 Figure Descriptions

   The figure descriptions are adequate and follow the accessibility guidelines.

 Recommendation (Round 1)

   I recommend Revise and Resubmit

 Review (Round 1)

   Thank you for your submission, I enjoyed reviewing your paper. You take up
               important, timely research questions on the understandability of
               privacy policies. I found your research questions to be original, and
               your methods sound and rigorous. It is great, for example, to have
               empirical work that shows which privacy concepts are “understandable”
               and your tables and descriptions show a great amount of detail.

   That being said, I do have a number of concerns (e.g. related works, discussion /
               implications) and presentation clarity that in the current state
               obstruct the impact of this work.

   Overall, I find that this paper could be written more clearly. It could use a few
               rounds of heavy copy editing to ensure a smoother flow.

   Next, I find that our paper is not sufficiently motivated in the introduction, nor
               sufficiently grounded adequately in prior work. For example, you
               present your research questions in the introduction without defining
               the research area — what is “understandability data”? What are the
               privacy concepts that ToSDR encompasses? Why is this your research
               site?

   Related Works:

   While your related works section does an adequate job of citing prior works - I
               find the organization unconvincing and the subsections scattered. It
               would strengthen your paper to rewrite this section with a better
               flow. For example, you start this section with {Websites profit off
               people’s trust by selling, sharing, or analyzing personal information
               [39]. As an example of the effects
   of these behaviors, “Slightly over half of participants (51%) felt that
               information about their general searching activities,...impacts their
               feelings about tracking.” [26] }. This does not read well. Summarizing
               the quote would be a better approach. Further as some more general
               writing tips, please use topic sentences and work on the transition
               flows between paragraphs and new ideas.

   Here are some more concrete suggestions towards a more organized structure for
               your related works section:

   1. Starting the section with an overview of a privacy theory or framework you are
               using and how you define privacy policies. You should ground these in
               related works in the HCI space.
   2. A subsection that starts with outlining the problem spaces concerning privacy
               policies (and then continuing with the other subsections you have).

   You cite the contextual integrity framework, which is fantastic. Along these
               lines, I would urge you to review this robust Zotero library for more
               work: https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.zotero.org%2Fgroups%2F2228317%2Fprivaci%2Flibrary&data=05%7C02%7Cjxd6067%40psu.edu%7C139527e5081d41ab9ca808dcfdeec6ca%7C7cf48d453ddb4389a9c1c115526eb52e%7C0%7C0%7C638664449203255851%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C0%7C%7C%7C&sdata=kuZvZm3fJMA%2FAtB4ogZvTzz3wauECQHegKaWaY0kpho%3D&reserved=0 but
               especially Shvartzshnaider et al., "Going against the (appropriate)
               flow: a contextual integrity approach to privacy policy analysis".

   Discussion / Implications

   Your findings and implications sections are quite muddled and it is very
               challenging to follow. I would highly recommend combing through these
               sections and trying to rewrite this for flow and readability.
               Importantly, throughout these sections, please cite prior work from
               your related works section. Here, you should be articulating how prior
               research informs (builds on, supports, or discounts, etc.) your
               empirical contributions -- this is crucial for having a paper with
               strong impact.

   I look forward to reviewing your edits. Good luck!

   Other specific edits:

   Introduction:

   Period missing at the end of second bullet point under “By answering these RQs, we
               make the following contributions”

   Methodology:

   Introduction is needed for ToSDR - what is ToSDR? Why ToSDR? What is the object or
               unit of analysis when scraping ToSDR?

   Period missing at the end of the last sentence in section 3.1 (Demographic
               information)

   Findings / Implications / Discussion:

   Period missing at the end of the last sentence in section 4.3

----------------------------------------------------------------



==> documentBody/a-leftovers.tex <==
\section{LEFTOVERS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Which privacy concepts received low severity ratings?}
\label{weakestSection}

Since the overall severity score was moderate to high, about 16\% of the responses had a severity score of less than 3 favoring either party, suggesting that participants viewed these case as largely unimportant.
In terms of the number of cases, 92 cases had a severity score of 3 or less favoring either party.
The following cases were perceived to be the least comprehensible (with an understandability score of 1) and least severe (with a severity score of 1 or -1):
\begin{itemize}
    \item \case{9}{An onion site accessible over Tor is provided}
    \item \case{15}{Content is published under a free license instead of a bilateral one}
    \item \case{44}{Minors must have the authorization of their legal guardians to use the service}
    \item \case{71}{The copyright license that you grant this service is limited to the parties that make up the service's broader platform.}
    \item \case{80}{The service claims to be CCPA compliant for California users}
    \item \case{82}{The service claims to be LGPD compliant for Brazilian users}
    \item \case{179}{You aren't allowed to remove or edit user-generated content}
    \item \case{192}{You can request access, correction and/or deletion of your data}
    \item \case{229}{Your personal data is aggregated into statistics}
    \item \case{146}{Tracking cookies refused will not limit your ability to use the service}
    \item \case{155}{very broad}
    \item \case{193}{You can scrape the site, as long as it doesn't impact the server too much}
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{How understandable are the least severe case?}
\label{sec:leastSevere}

Out of the 200 least severe responses (i.e., 1 and -1), only 51 responses were in favor of the Service Provider, leaving 149 favoring the User.
Out of those 51 responses that favored the Service Provider, 30 of them had the highest understandability score.

By contrast, in cases with the lowest severity score of 1, a total of 169 responses featured a maximum understandability score of 10.
This suggests that clarity is not necessarily impaired in situations that participants considered less severe.
Of the examples considered, 75 instances were in favor of the User, while 30 were in favor of the Service Provider.

The results indicate that although there is a prevailing pattern of strong comprehensibility being linked to severe consequences, there are individual cases that deviate from this pattern.
Although participants may have difficulty understanding certain cases, especially those that benefit the Service Provider, they may still perceive those cases as serious.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Summary}

%This analysis sheds light on the complex relationship between understandability and severity in the context of privacy policies.
%While high understandability often correlates with high perceived severity, particularly in Service Provider-favored cases, some participants may perceive cases as severe despite low understanding.
%The party favored also plays a key role in shaping perceptions, with Service Provider-favored cases being more likely to receive extreme severity ratings.
These insights highlight the importance of improving the clarity of privacy policies, particularly in cases where the stakes are high for users.







\subsection{How does this work help us in understanding/resolving the Privacy Paradox?}

\FIXME{R1-19: 10: The privacy paradox is discussed in the introduction, but never returned to. Why is this relevant?\\
JED@SNS: If you do not have a solid answer to R1-19 that is doable QUICKLY, we should make that paradox less primary to the motivation, since I think I have a decent argument I can develop QUICKLY for the other subsections here that should address R1-6.}









\subsection{what will exactly happen when the users are made aware of these policies?}

\FIXME{This needs to move to discussion since we are speculating a bit}

When users become more aware of privacy policies through the use of a tool that simplifies and clarifies them, several significant outcomes become possible.
Several enhancements or modifications may take place if businesses, legislators, and regulators learn about user interaction with privacy rules through this kind of study:

\begin{itemize}[nosep]
\item \textbf{Increased Awareness of Data Rights}: Users will become more knowledgeable about their rights regarding data privacy.
This includes understanding what data is being collected, how their data is being used, and what control they have.
Companies might simplify their privacy policies to make them more user-friendly.
Clear, concise, and transparent policies could become a competitive advantage.

\item \textbf{Empowered Decision-Making}: With a clear understanding of privacy terms, users can make more informed decisions about which services to use and what terms they are comfortable agreeing to allow.
This empowerment could lead to more selective consent, where users opt in or out based on their privacy preferences.

\item \textbf{Demand for Better Privacy Practices}: As public knowledge grows, there could be increased pressure on institutions (i.e., businesses or governments) to adopt or require more user-friendly privacy practices.
This could lead to more transparent data handling and potentially even influence legislative changes.
Companies might seek to collaborate more with privacy experts, legal advisors, and technology providers to improve their privacy policies and practices.

\item \textbf{Behavioral Changes in Digital Spaces}: With a better grasp of privacy implications, users might alter their behavior online, such as being more cautious about sharing personal information or using privacy-enhancing tools and settings.
The awareness of such an analysis in the think tank of the company can drive innovation, leading companies to develop new technologies and methods for protecting user privacy.
Increased awareness can also ensure better compliance with existing and emerging data protection regulations, thereby avoiding legal repercussions.

\item \textbf{Trust in Digital Services}:
By demonstrating a commitment to transparency and user privacy, companies can build greater trust with their customers, which is crucial for brand reputation and customer loyalty.
If companies respond positively by simplifying their privacy policies and respecting user preferences, this could lead to increased trust in these services.
Companies might reevaluate their data collection and processing practices, leading to more ethical and responsible use of user data.
Conversely, if users become aware of overly invasive or unfair practices, it could lead to a backlash against certain companies, prompting them to revise their policies.

\item \textbf{Rise in Demand for Privacy-Focused Services}: Awareness could drive demand for services and products that prioritize user privacy, potentially shifting market trends.
Companies may shift towards more user-centric approaches in handling personal data, including giving users more control over what data is collected and how it is used.

\item \textbf{More Informed and Far-Reaching Public Discourse on Privacy}: Awareness can stimulate public discourse on digital privacy, leading to a more informed public debate and potentially influencing policy decisions at the governmental level.

\end{itemize}












To resolve the privacy paradox, a comprehensive strategy is needed that includes boosting user education, streamlining privacy policies, and enhancing openness in data practices.


%Although there are exceptions, these results indicate that a low understandability score typically correlates with extremely negative perceived severity.
%A subset of participants acknowledge the potential importance of a case, especially when it favors the Service Provider, even if they have difficulty comprehending it.



%These advancements highlight that technology has the capacity to improve understanding and promote user involvement with rules, establishing a standard for clear and transparent digital communications.
%This automated tool will be in the form of a browser extension when upon opening any website's privacy policy or ToS document gives a summarized annotated version of the document for the user to read in a faster and efficient way.
%JED: commented out the above line. Why? we arent trying to propose tools here, just to use them as a motivation on why we need this data that we just collected.
%Addressing this issue through technological innovation not only enhances user empowerment and data literacy but also fosters a more ethically responsible digital environment.
%JED: commented out a line a bit above and also directly above. Why? not adding much. we made the point succinctly already

%An accurate analysis of the data and identification of trends or patterns relating to specific user groups can be achieved by comprehending the demographic profile of our participants.
%This demographic data will enable us to evaluate whether specific demographics have greater difficulty in comprehending privacy policies or perceive them as more stringent.
%JED: commented out hte above. Why? the first sentence says the same thing as the bottom commented line, but more succinctly. The top commented line just doesn't add much

%Through the integration of these inquiries, our objective is to reveal potential disparities among diverse user groups in terms of how consumers perceive and engage with privacy regulations.
%This information will be vital in developing privacy messages that are both inclusive and effective.
%JED: commented out the above. Why? not adding much. Just the facts, ma'am

%This also suggests that some participants considered the case to favor users while some considered it to favor the service providers. % Commented out because we make this point elsewhwere in a stronger way

%Recall that we gave participants access to both the succinct case label, as well as a lengthier paragraph giving more detail, also from \tosdr{}. %Commented out for brevity and it doesn;t really matter that much here anyway

\FIXED{
\begin{enumerate}
\item Identify Key barriers to policy understanding
    \subitem This survey systematically analyzes and identifies particular legal and policy concepts that consistently provide difficulties for users in understanding.
    \item Quantitative Insights into User Perception of Bias in Policy Favoritism
    \subitem  The finding, that two-thirds of the participants perceive a substantial tilt towards the Service Providers, adds to the debate on fairness and equality in policy development by presenting evidence of an imbalance in policy concepts that might impact user trust and consent.
    \item Legal Policy Reform Implications
    \subitem Through the identification of precise areas where user understanding is deficient, this research provides a basis for legislative reform initiatives that seek to streamline policy structure in order to promote more openness and justice in digital services.
    \item By measuring severity and understandability we seek to encompass both affective and cognitive reactions to privacy concepts. Our objective is to identify concepts participants (do not) value, as well as areas that suffer from lack of clarity.  The rewritten cases give the potential alternate text that we can use in place of ToSDR case labels that receive a low understandability rating.
    
\end{enumerate}}
